MEET: Mixture of Experts Extra Tree-Based sEMG Hand Gesture Identification

Artificial intelligence (AI) has made significant advances in recent years and opened up new possibilities in exploring applications in various fields such as biomedical, robotics, education, industry, etc. Among these fields, human hand gesture recognition is a subject of study that has recently emerged as a research interest in robotic hand control using electromyography (EMG). Surface electromyography (sEMG) is a primary technique used in EMG, which is popular due to its non-invasive nature and is used to capture gesture movements using signal acquisition devices placed on the surface of the forearm. Moreover, these signals are pre-processed to extract significant handcrafted features through time and frequency domain analysis. These are helpful and act as input to machine learning (ML) models to identify hand gestures. However, handling multiple classes and biases are major limitations that can affect the performance of an ML model. Therefore, to address this issue, a new mixture of experts extra tree (MEET) model is proposed to identify more accurate and effective hand gesture movements. This model combines individual ML models referred to as experts, each focusing on a minimal class of two. Moreover, a fully trained model known as the gate is employed to weigh the output of individual expert models. This amalgamation of the expert models with the gate model is known as a mixture of experts extra tree (MEET) model. In this study, four subjects with six hand gesture movements have been considered and their identification is evaluated among eleven models, including the MEET classifier. Results elucidate that the MEET classifier performed best among other algorithms and identified hand gesture movement accurately.

==> figure_tex/ablation.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{figure_pdf/ablation.pdf}
    \caption{\textbf{(Left) Orthogonal adaptation.} Enforcing row-space orthogonality between style and content LoRA improves image quality, where the images capture the style better and have fewer visual artifacts. \textbf{(Right) Style guidance.} We compare style control capabilities between our style guidance and standard LoRA weight scaling~\cite{dreamboothlora}. \textbf{{\color{MyDarkBlue} Blue}} and \textbf{{\color{MyDarkGreen} green}} stand for the LoRA weight scale and style guidance scale, respectively. Style guidance better preserves content when the style is applied. More details of style guidance formulation are in Section~\ref{sec:cfgstyle}.}
    \label{fig:ablation}
    \vspace{-10pt}
\end{figure}


==> figure_tex/baselines_style_guid.tex <==
\begin{figure*}[!t]
    \centering
    \includegraphics[width=\textwidth]{figure_pdf/baselines_style_guid.pdf}
    \caption{\maxwellchange{Result of our method compared to the strongest baselines, but replacing LoRA scale (Eq. \ref{eq:oldinference}) with our style guidance (Eq. \ref{eq:newinference}) for the baselines. While our style guidance increases baseline performance over LoRA scale images displayed in Figure \ref{fig:main_result}, our method is still superior in terms of preserving content while applying style.}}
    \label{fig:baseline_style_guid}
        \vspace{-10pt}

\end{figure*}


==> figure_tex/blending.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.95\linewidth]{figure_pdf/blending_v2.pdf}
        \vspace{-5pt}
    \caption{\textbf{Blending multiple style guidances.} We can compose multiple customized models by directly blending each style guidance together. Adjusting blending strength of each model allows us to acquire a smooth style transition. Train Image Pair 0 Style image credits: \href{https://www.instagram.com/parkhouse_art/}{Jack Parkhouse}}
    \label{fig:blending}
    \vspace{-10pt}
\end{figure}


==> figure_tex/limitation.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{figure_pdf/limitation.pdf}
    \caption{\textbf{Limitations.} \emph{Left}: 
     our method struggles with categories when they significantly differ from the training categories. Here, our method fails to transfer the artistic style of landscape image pairs to human portraits. \emph{Right}: our method can cause structure changes in some instances, like change of body position or background changes.
    }
    \label{fig:limitation}
    \vspace{-10pt}
\end{figure}


==> figure_tex/main_figure.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{figure_pdf/main_results_v7.pdf}
    \caption{Result of our method compared to the strongest baselines.
    \maxwellchange{When only training with the style image as in DB LoRA, the image structure is not preserved and overfitting occurs. While Concept Slider's training scheme~\cite{gandikota2023concept} uses both style and content images, it still exhibits overfitting and loss of structure in many cases.} Our method preserves the structure of the input mage while faithfully applying the desired style. We use style guidance strength 3 and classifier guidance strength 5.
    Style image credits: \href{https://www.instagram.com/parkhouse_art/}{Jack Parkhouse} (Third row) and \href{https://www.instagram.com/aaronhertzmann/?hl=en}{Aaron Hertzmann} (Fourth row)}
    \label{fig:main_result}
\end{figure*}


==> figure_tex/method.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=\linewidth]{figure_pdf/method_v7.pdf}
        \vspace{-5pt}
    \caption{\textbf{Method overview}. (Left) We disentangle style and content from an image pair by jointly training two low-rank adapters, StyleLoRA and ContentLoRA, representing style and content, respectively. Our training objective consists of two losses: The first loss fine-tunes ContentLoRA to reconstruct content image conditioned on a content prompt. The second loss encourages reconstructing the style image using \textit{both} StyleLoRA and ContentLoRA conditioned on a style prompt, but we only optimize Style LoRA for this loss. (Right) At inference time, we only apply StyleLoRA to customize the model. Given the same noise seed, the customized model generates a stylized counterpart of the original pre-trained model output. {\menlo V*} is a fixed random rare token that is a prompt modifier for the content image. Style image credits: \href{https://www.instagram.com/parkhouse_art/}{Jack Parkhouse}}
    \label{fig:method}
        \vspace{-10pt}
\end{figure*}



==> figure_tex/mturk.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=.7\textwidth]{figure_pdf/turk_image.pdf}
    \caption{Mturk User Interface
    }

    \label{fig:mturk}
        \vspace{-10pt}
\end{figure}


==> figure_tex/teaser.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figure_pdf/teaser_jack_dog_v2.pdf}
        \vspace{-5pt}
    \caption{%
    Given a \emph{single} image pair, we present \methodname, a method for customizing a pre-trained text-to-image model and learning a new style from the image pair's stylistic difference. Our method can apply the learned stylistic difference to new input images while preserving the input structure. Compared to Dreambooth LoRA\cite{hu2022lora, loraimplementation}, a standard customization method that solely use style images, our method effectively disentangles style and content, resulting in better structure, color preservation, and style application. Style image credit: \href{https://www.instagram.com/parkhouse_art/}{Jack Parkhouse}.
    }
    \label{fig:teaser}
        \vspace{-15pt}
\end{figure*}



==> figure_tex/tradeoff_plot.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=\linewidth]{figure_pdf/quantitative_analysis_sliders.pdf}
    \caption{\textbf{Quantitative comparison with baselines on learned style.} Given a fixed inference path, our method's pareto dominates baselines for image generation both on the same category as training (left) and when evaluated on categories different from training, e.g., trained on human portraits but tested on dog images (right). \maxwellchange{Secondly, our proposed style guidance outperforms standard LoRA weight scale guidance for our training method (blue vs. orange), DB LoRA (green vs. pink), and Sliders (brown vs. purple)}. In the Appendix's Figure \ref{fig:tradeoff_plot_diversity}, we further evaluate the diversity of generated images. We show that baselines often lose diversity, while our method leads to diverse generations while still achieving lower perceptual distance to the ground truth style.
    Increased marker size corresponds to an increase in style guidance scale.
    }
    \label{fig:tradeoff_plot}
\end{figure*} 






==> figure_tex/tradeoff_plot_diversity.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.95\linewidth]{figure_pdf/sliders_diversity.pdf}
    \caption{\textbf{Quantitative comparison on Diversity metric.} Our method with style guidance has high diversity and low perceptual distance to ground truth style images both on the same category as training (left) and when evaluated on categories different from training, e.g., trained on human portraits but tested on dog images (right). 
    Methods without edge control tend to lose diversity indicating overfitting, and methods with edge control have similar/higher diversity, but much worse style application.  
    Increased marker size corresponds to an increase in style guidance scale.
    }
    \label{fig:tradeoff_plot_diversity}
\end{figure*} 






==> figure_tex/tradeoff_plot_diversity_style_aligned.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.95\linewidth]{figure_pdf/tradeoff_plot_diversity_style_aligned.pdf}
    \caption{\textbf{Image diversity with Style Aligned \cite{hertz2023style} on learned style (Diversity).} Our method has high diversity and low perceptual distance to ground truth style images both on the same category as training (left) and when evaluated on categories different from training, e.g., trained on human portraits but tested on dog images (right) as compared to both versions of Style Aligned Image Generation. 
    }
    \label{fig:tradeoff_plot_diversity_style_aligned}
\end{figure*} 






==> figure_tex/tradeoff_plot_style_aligned.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.95\linewidth]{figure_pdf/tradeoff_plot_style_aligned.pdf}
    \caption{\textbf{Style similarity with Style Aligned \cite{hertz2023style}.} Our method Pareto dominates both versions of Style Aligned Image Generation for image generation both on the same category as training (left) and when evaluated on categories different from training, e.g., trained on human portraits but tested on dog images (right).
    }
    \label{fig:tradeoff_plot_style_aligned}
\end{figure*} 






==> figure_tex/training_data.tex <==
\begin{figure*}[!t]
    \centering
    \includegraphics[width=\textwidth]{figure_pdf/training_data.pdf}
    \caption{\textbf{Training Data.} We present the synthetic training data set used for evaluation, where each pair is used as a single training instance. Each column corresponds to a different style, and each row corresponds to a different content category.}
    \label{fig:training_data}
\end{figure*}

